Lucy: Think and Reason to Solve Text-to-SQL

Large Language Models (LLMs) have made significant progress in assisting users to query databases in natural language. While LLM-based techniques provide state-of-the-art results on many standard benchmarks, their performance significantly drops when applied to large enterprise databases. The reason is that these databases have a large number of tables with complex relationships that are challenging for LLMs to reason about. We analyze challenges that LLMs face in these settings and propose a new solution that combines the power of LLMs in understanding questions with automated reasoning techniques to handle complex database constraints. Based on these ideas, we have developed a new framework that outperforms state-of-the-art techniques in zero-shot text-to-SQL on complex benchmarks

==> 101_prompt.tex <==
\subsection{Prompts description}
\input{prompts/promptA}
\input{prompts/promptC}


==> 20_background.tex <==
\section{Background}
We briefly overview relevant concepts (\cref{a:s:backgroud} gives an extended version).
%\noindent\textbf{Relational databases.}
A relation or table is defined as a set of tuples over attributes $X$. Projection is a unary operation on a subset of attribute  $Y \subseteq X$. The result of the projection is the set of tuples that is obtained when all tuples in \tbl are restricted to attributes $Y$. 
Inner join, or simply $\jn$, is a binary operator between tables $\tbl_1$ and $\tbl_2$ over their common attributes $Y$ that returns a set of all combinations of tuples in $\tbl_1$ and $\tbl_2$  that are equal on $Y$. Left join is similar to the join but returns all rows of $\tbl_1$ filling unmatched rows of $\tbl_2$ with null values.
%
A database can support a large set of constraints over tables. The two main constraint types are on primary and foreign keys that define relationships between tables.
A database typically represents entities and their interactions in real-world processes, e.g., the financial management of a company. To effectively model these entities, several design patterns have been developed~\citep{dimensional,patternsbook}. For example, a many-to-one pattern (\manyone) specifies a relationship when any number of attributes from one table is associated with unique attributes of the same or another table, enforced by foreign key and primary key relationships.  The \lookup table is a table that contains description values used by multiple tables, e.g., zip codes. A \stars pattern is a type of relational database schema composed of a single, central fact table surrounded by dimension tables. A \snow schema consists of one fact table connected to many dimension tables, which can be connected to other dimension tables through a many-to-one relationship.



==> exps/bird_table.tex <==
                \begin{table} 
                \scriptsize                \centering 
                 \begin{tabular}{|l|r|r|r|r|r|r|}
\hline 
 &\gptfour&\gptfourT&\gptfourTS&\chatfour&\nsql&\sys\\ 
 \hline 
\hline 
\hline 
$\cover_\tbl$ & 0.86 & 0.78 & 0.77 & 0.88 & 0.52 & 0.93 \\ 
 \hline 
$\cover_\att$ & 0.84 & 0.75 & 0.75 & 0.81 & 0.50 & 0.94 \\ 
 \hline 
$\ex$ & 54 & 67 & 65 & 80 & 9 & 83 \\ 
 \hline 
$\esx$ & 66 & 80 & 79 & 93 & 10 & 103 \\ 
 \hline 
                \end{tabular}                \caption{\label{tab:formula_1_gt-corrected} Results for the \formula dataset.} 
                \end{table}                \begin{table} 
                \scriptsize                \centering 
                 \begin{tabular}{|l|r|r|r|r|r|r|}
\hline 
 &\gptfour&\gptfourT&\gptfourTS&\chatfour&\nsql&\sys\\ 
 \hline 
\hline 
\hline 
$\cover_\tbl$ & 0.81 & 0.84 & 0.87 & 0.92 & 0.50 & 0.99 \\ 
 \hline 
$\cover_\att$ & 0.81 & 0.81 & 0.85 & 0.91 & 0.59 & 0.96 \\ 
 \hline 
$\ex$ & 36 & 47 & 52 & 59 & 6 & 56 \\ 
 \hline 
$\esx$ & 38 & 55 & 64 & 62 & 6 & 68 \\ 
 \hline 
                \end{tabular}                \caption{\label{tab:financial_gt-corrected} Results for the \financial dataset.} 
                \end{table}

==> exps/insurance_table.tex <==
                \begin{table} 
                \scriptsize                \centering 
                 \begin{tabular}{|l|r|r|r|r|r|r|r|}
\hline 
 &\gptfourT&\gptfourTS&\chatfour&\nsql&\sys\\ 
 \hline 
\hline 
\hline 
$\cover_\tbl$ & 0.44 & 0.47 & 0.82 & 0.31 & 0.95 \\ 
 \hline 
$\cover_\att$ & 0.36 & 0.42 & 0.81 & 0.25 & 0.93 \\ 
 \hline 
$\ex$ & 9 & 13 & 16 & 2 & 30 \\ 
 \hline 
$\esx$ & 9 & 13 & 16 & 3 & 33 \\ 
 \hline 
                \end{tabular}                \caption{\label{tab:insurance_gt} Results for the \insurance dataset.} 
                \end{table}



==> exps/vsphere_large_table.tex <==
                \begin{table} 
                \scriptsize                \centering 
                 \begin{tabular}{|l|r|r|r|r|r|r|r|}
\hline 
 &\gptfourT&\gptfourTS&\chatfour&\sys\\ 
 \hline 
\hline 
\hline 
$\cover_\tbl$ & 0.46 & 0.44 & 0.44 & 0.98 \\ 
 \hline 
$\cover_\att$ & 0.50 & 0.44 & 0.48 & 0.98 \\ 
 \hline 
$\ex$ & 6 & 4 & 2 & 17 \\ 
 \hline 
$\esx$ & 9 & 5 & 2 & 18 \\ 
 \hline 
                \end{tabular}                \caption{\label{tab:vsphere_large_gt} Results for the \vlarge dataset.} 
                \end{table}

==> figures/trees.tex <==
\tikzstyle{startstop} = [rectangle, rounded corners, 
minimum width=1cm, 
minimum height=0.5cm,
text centered, 
draw=black, 
fill=white!20]

\tikzstyle{data} = [rectangle, rounded corners, 
minimum width=1.7cm, 
minimum height=1cm,
text width=4em,
text centered, 
draw=white, 
fill=white!30]


\tikzstyle{smalldata} = [rectangle, rounded corners, 
minimum width=0.1cm, 
minimum height=0.2cm,
text width=2em,
text centered, 
draw=white, 
fill=white!30]
\tikzstyle{io} = [trapezium, 
trapezium stretches=true, % A later addition
trapezium left angle=70, 
trapezium right angle=110, 
minimum width=3cm, 
minimum height=1cm, text centered, 
draw=black, fill=blue!30]

\tikzstyle{process} = [rectangle, 
minimum width=0.2cm, 
minimum height=1cm, 
text centered, 
text width=4em,
draw=black,dashed, 
fill=gray!10]

\tikzstyle{processsmall} = [rectangle, 
minimum width=0.2cm, 
minimum height=1cm, 
text centered, 
text width=3em,
draw=black,dashed, 
fill=gray!10]

\tikzstyle{processbiga} = [rectangle,
 rounded corners, 
minimum width=2.8cm, 
minimum height=1.8cm, 
text centered, 
text width=5em,
draw=white, 
fill=white!10]

\tikzstyle{processbigb} = [rectangle,
 rounded corners, 
minimum width=5.1cm, 
minimum height=1.8cm, 
text centered, 
text width=5em,
draw=white, 
fill=white!20]
\tikzstyle{processbigc} = [rectangle,
 rounded corners, 
minimum width=6.9cm, 
minimum height=2.2cm, 
text centered, 
text width=5em,
draw=white, 
fill=white!10]
\tikzstyle{decision} = [diamond, 
minimum width=3cm, 
minimum height=1cm, 
text centered, 
draw=white, 
fill=white!30]
\tikzstyle{arrow} = [thick,->,>=stealth]
\tikzstyle{line}     = [draw=black,thick]



% \node (dec1) [decision, below of=pro1, yshift=-0.5cm] {Decision 1};

% \node (pro2a) [process, below of=dec1, yshift=-0.5cm] {Process 2a
% text text text text
% text text text 
% text text text};

% \node (pro2b) [process, right of=dec1, xshift=2cm] {Process 2b};
% \node (out1) [io, below of=pro2a] {Output};
\begin{figure}
\centering

\begin{tikzpicture}[auto, node distance=2cm, every node/.style={sloped}]
\node (pam) [startstop, font=\small]{\pam};
\node (client) [startstop, font=\small, right of=pam]{\client};
\node (loc) [startstop, font=\small, right of=client, xshift= 0.8cm]{\loc};
\node (dc) [startstop, font=\small, right of=loc, xshift= 0.8cm]{\dc};
\node (compute) [startstop, font=\small, right of=dc, xshift= 0.8cm]{\compres};
\node (pama) [startstop, font=\small, below of=pam,yshift= 1cm]{\pama};
\node (tax) [startstop, font=\small, below of=pama, xshift= -2.4cm,yshift= 1cm]{\tax};
\node (charge) [startstop, font=\small, below of=pama, xshift= -0.6cm,yshift= 1cm]{\charge};
\node (income) [startstop, font=\small, below of=pama, xshift= +1.4cm,yshift= 1cm]{\income};
\node (retention) [startstop,font=\small, xshift= 1.7cm, right of=pama]{Retention};
\node (gift) [startstop, font=\small, below of=retention, xshift= -0.8cm,yshift= 1cm]{\gift};
\node (bonus) [startstop, font=\small, below of=retention, xshift= 0.6cm,yshift= 1cm]{\bonus};

\node (pool) [startstop, font=\small, below of=dc, xshift= 1.3cm, yshift= 1.3cm]{\respool};
\node (config) [startstop, font=\small, below of=pool, xshift= -2.0cm, yshift= 1.4cm]{\config};
\node (runtime) [startstop, font=\small, below of=pool, xshift= 1.6cm, yshift= 1.4cm]{\runtime};
\node (cmem) [startstop, font=\small, below of=config, xshift= -0.8cm, yshift= 1.4cm]{\cmem};
\node (ccpu) [startstop, font=\small, below of=config, xshift= 0.8cm, yshift= 1.4cm]{\ccpu};
\node (rmem) [startstop, font=\small, below of=runtime, xshift= -0.8cm, yshift= 1.4cm]{\rmem};
\node (rcpu) [startstop, font=\small, below of=runtime, xshift= 0.8cm, yshift= 1.4cm]{\rcpu};
\begin{scope}[on background layer]
\node (stara) [processbiga, font=\small, below of=retention, xshift= -0.1cm, yshift= 1.5cm, label=below:Star A]{};
\end{scope}
\begin{scope}[on background layer]
\node (starb) [processbigb, font=\small, below of=pama, xshift= -0.4cm, yshift= 1.5cm, label=below:Star B]{};
\end{scope}

\begin{scope}[on background layer]
\node (starb) [processbigc, font=\small, below of=pool, xshift= -0.4cm, yshift= 1.3cm, label=below:Snowflake]{};
\end{scope}



\draw [line] (retention) --  (gift);
\draw [line] (retention) --  (bonus);
\draw[thick,black](pama) --  (tax);
\draw[thick,black] (pama) --  (charge);
\draw[thick,black] (pama) --  (income);
\draw [line] (pool) --  (config);
\draw [line] (pool) --  (runtime);
\draw [line] (config) --  (cmem);
\draw [line] (config) --  (ccpu);
\draw [line] (runtime) --  (rmem);
\draw [line] (runtime) --  (rcpu);

% \node (retrieve) [startstop, right of=input1, xshift= 0.5cm] {Retrieve};
% %\node (output1) [data, right of=retrieve, xshift= 0.3cm] {\client, \\ \dc};
% \node (solveoverall) [processbig, right of=retrieve, xshift=2.8cm, label=below:Generate(constraint reasoning)] {};
% \node (solve) [processsmall, right of=retrieve, xshift=1.0cm] {Solve};
% %\node (output2) [smalldata, right of=solve, xshift= 0.01cm] {Path};
% \node (view) [process, right of=solve, xshift= 1.5cm] {Generate \\ view};
% \node (sql) [startstop, right of=view, xshift=1.2cm] {TvS};




% \node (pro2) [process, right of=pro1, xshift= 2.5cm] {View};
% \node (pro3) [startstop, right of=pro2, xshift= 2.5cm] {SQL};
%\node (stop) [startstop, below of=out1] {Stop};
% \draw [arrow] (input1)to[right] node[anchor=south] {} (retrieve);
% %\draw [arrow] (-0.3,-0.3)to[right] node[anchor=north] {\scriptsize{\dbm}} (retrieve);

% %\draw [arrow] (input1) --  (retrieve);
% \draw [arrow] (retrieve) --   node [above] {\scriptsize{Relevant}} node [below] {\scriptsize{tables}}  (solve) ;
% %\draw [arrow] (output1) -- (solve);
% \draw [arrow] (solve) --   node [above] {\scriptsize{Path between}} node [below] {\scriptsize{relevant tables}} (view);
% %\draw [arrow] (input1)to[right] node[anchor=north] {\scriptsize{Question}} (sql);
% %\draw [arrow] (9.8,-0.5)to[right] node[anchor=north] {\scriptsize{Question}} (sql);
% \draw [arrow] (view) --  node [above] {\scriptsize{Summary}}   node [below] {\scriptsize{view}}  (sql);
% \draw [arrow] (sql) to[right] node[auto] {\scriptsize{SQL}} ++ (1.7,0);
% \path[line] (input1.south) -- +(0,-1) -|  (sql.south) node[pos=0.25,below]{} ;  
% \path[line] (input0.east) -- +(0,0) -|  (sql.north) node[pos=0.25,above]{} ;  
% \path[line] (input0.east) -- +(0,0) -|  (solve.north) node[pos=0.25,above]{} ;  
% \path[line] (input0.east) -- +(0,0) -|  (view.north) node[pos=0.25,above]{} ;  

% \path[line] (input0.east) -- +(0,0) -|  (retrieve.north) node[pos=0.25,above]{} ;  

% \path[line] (input0.north) -- +(0,-1) -|  (solveoverall.north) node[pos=0.25,below]{} ;  
% \path[line] (input0.north) -- +(0,-1) -|  (retrieve.north) node[pos=0.25,below]{} ;  
\end{tikzpicture}
\caption{Tree decomposition} \label{fig:trees}
\end{figure}
